Adversarial Network Traffic: Towards Evaluating the Robustness of Deep Learning-Based Network Traffic Classification

Network traffic classification is used in various applications such as network traffic management, policy enforcement, and intrusion detection systems. Although most applications encrypt their network traffic and some of them dynamically change their port numbers, Machine Learning (ML) and especially Deep Learning (DL)-based classifiers have shown impressive performance in network traffic classification. In this paper, we evaluate the robustness of DL-based network traffic classifiers against Adversarial Network Traffic (ANT). ANT causes DL-based network traffic classifiers to predict incorrectly using Universal Adversarial Perturbation (UAP) generating methods. Since there is no need to buffer network traffic before sending ANT, it is generated live. We partition the input space of the DL-based network traffic classification into three categories: packet classification, flow content classification, and flow time series classification. To generate ANT, we propose three new attacks injecting UAP into network traffic. AdvPad attack injects a UAP into the content of packets to evaluate the robustness of packet classifiers. AdvPay attack injects a UAP into the payload of a dummy packet to evaluate the robustness of flow content classifiers. AdvBurst attack injects a specific number of dummy packets with crafted statistical features based on a UAP into a selected burst of a flow to evaluate the robustness of flow time series classifiers. The results indicate injecting a little UAP into network traffic, highly decreases the performance of DL-based network traffic classifiers in all categories.

==> content/Apendix_A.tex <==



\begin{table}[H]
	\caption{
		The architecture (A) and hyperparameters (B) of 1D-CNN packet classifiers PC-HP, and PC-P.}
	\label{tab:PC_selected_arch}
	\begin{minipage}{.5\linewidth}
		\caption*{(A)}
		\centering
	\resizebox{6cm}{!}{%
	\begin{tabular}{|
			>{\columncolor[HTML]{EFEFEF}}c |c|c|}
		\hline
		\# & \cellcolor[HTML]{EFEFEF}Layer & \cellcolor[HTML]{EFEFEF}Parameters \\ \hline
		1 & 1D-Convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 256, \\ Filter size: 4,\\ Strides: 2\end{tabular} \\ \hline
		2 & Batch normalization & - \\ \hline
		3 & Relu & - \\ \hline
		4 & 1D-Convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 128, \\ Filter size: 8, \\ Stride: 2\end{tabular} \\ \hline
		5 & Batch Normalization & - \\ \hline
		6 & Relu & - \\ \hline
		7 & 1D-Max Polling & \begin{tabular}[c]{@{}c@{}}Filter size: 2,\\ Strides: 1\end{tabular} \\ \hline
		8 & Dense & Size: 256 \\ \hline
		9 & Batch normalization & - \\ \hline
		10 & Relu & - \\ \hline
		11 & Dropout & Rate: 0.1 \\ \hline
		12 & Dense & Size: 128 \\ \hline
		13 & Batch normalization & - \\ \hline
		14 & Relu & - \\ \hline
		15 & Dropout & Rate: 0.1 \\ \hline
		16 & Dense & Size: 6 \\ \hline
		17 & Softmax & - \\ \hline
	\end{tabular}
}
	\end{minipage}%
	\begin{minipage}{.5\linewidth}
		\centering
		\caption*{(B)}
	\resizebox{6cm}{!}{%
	\begin{tabular}{|c|c|}
	\hline
	\rowcolor[HTML]{EFEFEF} 
	Hyperparameter & Value \\ \hline
	Optimizer & Adamax \\ \hline
	Learning rate & 0.0005 \\ \hline
	Batch size & 128 \\ \hline
	Epoch number & 1000 \\ \hline
	Validation metric & Accuracy \\ \hline
	DL framework & Tensorflow \& Keras \\ \hline
	\end{tabular}
}
	\end{minipage} 
\end{table}

\begin{table}[H]
	\caption{The architecture (A) and hyperparameters (B) of 1D-CNN flow content classifiers FCC-HP, and FCC-P.}
	\label{tab:FCC_selected_arch}
	\begin{minipage}{.5\linewidth}
		\caption*{(A)}
		\centering
	\resizebox{10cm}{!}{%
	\begin{tabular}{|
		>{\columncolor[HTML]{EFEFEF}}c |c|c|
		>{\columncolor[HTML]{EFEFEF}}c |c|c|}
	\hline
	\# & \cellcolor[HTML]{EFEFEF}Layer & \cellcolor[HTML]{EFEFEF}Parameters & \# & \cellcolor[HTML]{EFEFEF}Layer & \cellcolor[HTML]{EFEFEF}Parameters \\ \hline
	1 & 1D-convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 32\\ Filter size: 4\\ Strides: 1\end{tabular} & 17 & Dense & Size: 512 \\ \hline
	2 & Elu & Alpha: 1.0 & 18 & Batch normalization &-  \\ \hline
	3 & Batch normalization & - & 19 & Relu &-  \\ \hline
	4 & 1D-Max pooling & \begin{tabular}[c]{@{}c@{}}Filter size: 8\\ Strides: 2\end{tabular} & 20 & Dropout & Rate: 0.05 \\ \hline
	5 & 1D-convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 64\\ Filter size: 4\\ Strides: 1\end{tabular} & 21 & Dense & Size: 512 \\ \hline
	6 & Elu & Alpha: 1.0 & 22 & Batch normalization &-  \\ \hline
	7 & Batch normalization &-& 23 & Relu &-  \\ \hline
	8 & 1D-Max pooling & \begin{tabular}[c]{@{}c@{}}Filter size: 8\\ Strides: 2\end{tabular} & 24 & Dropout & Rate: 0.05 \\ \hline
	9 & 1D-convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 128\\ Filter size: 8\\ Strides: 1\end{tabular} & 25 & Dense & Size: 6 \\ \hline
	10 & Elu & Alpha: 1.0 & 26 & Softmax & - \\ \hline
	11 & Batch normalization & -&  &  &  \\ \hline
	12 & 1D-Max pooling & \begin{tabular}[c]{@{}c@{}}Filter size: 8\\ Strides: 2\end{tabular} &  &  &  \\ \hline
	13 & 1D-convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 256\\ Filter size: 8\\ Strides: 1\end{tabular} &  &  &  \\ \hline
	14 & Elu & Alpha: 1.0 &  &  &  \\ \hline
	15 & Batch normalization &-  &  &  &  \\ \hline
	16 & 1D-Max pooling & \begin{tabular}[c]{@{}c@{}}Filter size: 8\\ Strides: 2\end{tabular} &  &  &  \\ \hline
	\end{tabular}
	}
	\end{minipage}%
	\begin{minipage}{.5\linewidth}
		\raggedleft
		\caption*{\quad\quad\quad\quad\quad\quad(B)}
		\resizebox{6cm}{!}{%
	\begin{tabular}{|c|c|}
	\hline
	\rowcolor[HTML]{EFEFEF} 
	Hyperparameter & Value \\ \hline
	Optimizer & Adamax \\ \hline
	Learning rate & 0.0005 \\ \hline
	Batch size & 128 \\ \hline
	Epoch number & 1000 \\ \hline
	Validation metric & Accuracy \\ \hline
	DL framework & Tensorflow \& Keras \\ \hline
	\end{tabular}
	}
	\end{minipage} 
\end{table}




\begin{table}[H]
	\caption{The architecture (A) and hyperparameters (B) of 1D-CNN flow time series classifiers, FTSC-PS, and FTSC-IAT.}
	\label{tab:FTSC-arch}
	\begin{minipage}{.5\linewidth}
		\caption*{(A)}
		\centering
\resizebox{10cm}{!}{%
	\begin{tabular}{|
			>{\columncolor[HTML]{EFEFEF}}c |c|c|
			>{\columncolor[HTML]{EFEFEF}}c |c|c|}
		\hline
		\# & \cellcolor[HTML]{EFEFEF}Layer & \cellcolor[HTML]{EFEFEF}Parameters & \# & \cellcolor[HTML]{EFEFEF}Layer & \cellcolor[HTML]{EFEFEF}Parameters \\ \hline
		1 & 1D-Convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 128, \\ Filter size: 16,\\ Strides: 1\end{tabular} & 22 & 1D-Convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 256, \\ Filter size: 4,\\ Strides: 1\end{tabular} \\ \hline
		2 & Elu & Alpha: 1.0 & 23 & Elu & Alpha: 1.0 \\ \hline
		3 & Batch normalization & - & 24 & Batch normalization & - \\ \hline
		4 & 1D-Convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 128, \\ Filter size: 16, \\ Stride: 1\end{tabular} & 25 & 1D-Convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 256, \\ Filter size: 4,\\ Strides: 1\end{tabular} \\ \hline
		5 & Elu & Alpha: 1.0 & 26 & Elu & Alpha: 1.0 \\ \hline
		6 & Batch Normalization & - & 27 & Batch Normalization & - \\ \hline
		7 & 1D-Max Polling & \begin{tabular}[c]{@{}c@{}}Filter size: 4,\\ Strides: 2\end{tabular} & 28 & 1D-Max Polling & \begin{tabular}[c]{@{}c@{}}Filter size: 4,\\ Strides: 2\end{tabular} \\ \hline
		8 & 1D-Convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 128, \\ Filter size: 8,\\ Strides: 1\end{tabular} & 29 & Dense & Size: 1024 \\ \hline
		9 & Elu & Alpha: 1.0 & 30 & Batch normalization & - \\ \hline
		10 & Batch normalization & - & 31 & Relu & - \\ \hline
		11 & 1D-Convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 128, \\ Filter size: 8,\\ Strides: 1\end{tabular} & 32 & Dropout & Rate: 0.05 \\ \hline
		12 & Elu & Alpha: 1.0 & 33 & Dense & Size: 512 \\ \hline
		13 & Batch Normalization & - & 34 & Batch normalization & - \\ \hline
		14 & 1D-Max Polling & \begin{tabular}[c]{@{}c@{}}Filter size: 4,\\ Strides: 2\end{tabular} & 35 & Relu & - \\ \hline
		15 & 1D-Convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 128, \\ Filter size: 4,\\ Strides: 1\end{tabular} & 36 & Dropout & Rate: 0.05 \\ \hline
		16 & Elu & Alpha: 1.0 & 37 & Dense & Size: 512 \\ \hline
		17 & Batch normalization & - & 38 & Batch normalization & - \\ \hline
		18 & 1D-Convolution & \begin{tabular}[c]{@{}c@{}}Number of filters: 128, \\ Filter size: 4,\\ Strides: 1\end{tabular} & 39 & Relu & - \\ \hline
		19 & Elu & Alpha: 1.0 & 40 & Dropout & Rate: 0.05 \\ \hline
		20 & Batch Normalization & - & 41 & Dense & Size: 6 \\ \hline
		21 & 1D-Max Polling & \begin{tabular}[c]{@{}c@{}}Filter size: 4,\\ Strides: 2\end{tabular} & 42 & Softmax & - \\ \hline
	\end{tabular}
}
	\end{minipage}%
	\begin{minipage}{.5\linewidth}
		\raggedleft
		\caption*{\quad\quad\quad\quad\quad\quad(B)}
		\resizebox{6cm}{!}{%
	\begin{tabular}{|c|c|}
	\hline
	\rowcolor[HTML]{EFEFEF} 
	Hyperparameter & Value \\ \hline
	Optimizer & Adamax \\ \hline
	Learning rate & 0.0003 \\ \hline
	Batch size & 128 \\ \hline
	Epoch number & 1000 \\ \hline
	Validation metric & Accuracy \\ \hline
	DL framework & Tensorflow \& Keras \\ \hline
	\end{tabular}
	}
	\end{minipage} 
\end{table}


\begin{table}[H]
	\centering
	\caption{(A) The overall accuracy of flow content classifiers for different number of packets in the byte sequence of each flow. (B) The overall accuracy of flow time series classifiers for different number of packets in the time series of each flow. }
	\label{tab:num_of_pkt_for_classification}
	\begin{minipage}{.5\linewidth}
		\caption*{(A)}
		\centering
		\begin{tabular}{|
				>{\columncolor[HTML]{EFEFEF}}c |c|c|}
			\hline
			\cellcolor[HTML]{EFEFEF} & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}Overall Accuracy(\%)} \\ \cline{2-3} 
			\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Num of Pkts in flow byte \\ sequence of each flow\end{tabular}} & \cellcolor[HTML]{EFEFEF}FCC-HP & \cellcolor[HTML]{EFEFEF}FCC-P \\ \hline
			7 & 79.25 & 78.50 \\ \hline
			10 & 81.52 & 80.6 \\ \hline
			12 & 80.38 & 79.61 \\ \hline
			15 & 81.50 & 79.72 \\ \hline
			17 & 79.95 & 78.08 \\ \hline
			20 & 80.31 & 78.26 \\ \hline
		\end{tabular}
	\end{minipage}%
	\begin{minipage}{.5\linewidth}
		\centering
		\caption*{(B)}
		\begin{tabular}{|
				>{\columncolor[HTML]{EFEFEF}}c |c|c|}
			\hline
			\cellcolor[HTML]{EFEFEF} & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}Overall Accuracy(\%)} \\ \cline{2-3} 
			\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Num of Pkts in \\ time series of each flow\end{tabular}} & \cellcolor[HTML]{EFEFEF}FTSC-PS & \cellcolor[HTML]{EFEFEF}FTSC-IAT \\ \hline
			10 & 71.94 & 72.5 \\ \hline
			25 & 74.73 & 74.09 \\ \hline
			50 & 74.26 & 75.02 \\ \hline
			75 & 75.38 & 76.16 \\ \hline
			100 & 76.21 & 76.51 \\ \hline
			250 & 75.56 & 76.79 \\ \hline
			500 & 75.66 & 75.77 \\ \hline
			750 & 76.12 & 75.11 \\ \hline
			1000 & 74.73 & 74.95 \\ \hline
		\end{tabular}
	\end{minipage} 
\end{table}




==> content/Apendix_D.tex <==
\newcommand{\FTSCchatp}{FTSC_cls_chat_precision.csv}
\newcommand{\FTSCemailp}{FTSC_cls_email_precision.csv}
\newcommand{\FTSCfilep}{FTSC_cls_filetransfer_precision.csv}
\newcommand{\FTSCstreamingp}{FTSC_cls_streaming_precision.csv}
\newcommand{\FTSCtorrentp}{FTSC_cls_torrent_precision.csv}
\newcommand{\FTSCvoipp}{FTSC_cls_voip_precision.csv}

\newcommand{\FTSCchatf}{FTSC_cls_chat_f_score.csv}
\newcommand{\FTSCemailf}{FTSC_cls_email_f_score.csv}
\newcommand{\FTSCfilef}{FTSC_cls_filetransfer_f_score.csv}
\newcommand{\FTSCstreamingf}{FTSC_cls_streaming_f_score.csv}
\newcommand{\FTSCtorrentf}{FTSC_cls_torrent_f_score.csv}
\newcommand{\FTSCvoipf}{FTSC_cls_voip_f_score.csv}

\begin{figure}[H]
	\centering
	
	\begin{tikzpicture}
	%/*
	\pgfplotsset{
		scaled y ticks = false,
		width=5cm,
		height=4cm,
		axis on top,
		%xticklabel style={text width=2em,align=center},
		%xticklabels={\empty},
		xmin=-1,xmax=21,
		ymin=-0,ymax=100,
		minor y tick num=1,
		xtick={1,3,5,7,10,12,15,17,20},
		ticklabel style = {font=\tiny},
		%xminorticks=true,
		%yminorticks=true,
		ylabel shift={-0.8em},
		ylabel style={align=center},
		xlabel shift={-0.4em},
		grid=both, 
		grid style={dashed,gray!30}
	}
	%       
	\begin{groupplot}[ 
	group style={
		group size=3 by 2,
		vertical sep=45pt,
		horizontal sep=35pt
	},
	]
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={Precision(\%)},title={Chat},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCPS\FTSCchatp};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCPS\FTSCchatp};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCPS\FTSCchatp};  
	
	% (Relative) Coordinate at top of the first plot
	\coordinate (c1) at (rel axis cs:0,1);
	
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={Precision(\%)},title={Email}]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCPS\FTSCemailp};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCPS\FTSCemailp};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCPS\FTSCemailp};  
	
	
	\nextgroupplot[
	yshift=0pt,
	xlabel={Num\_of\_Dummy\_Pkts},ylabel={Precision(\%)},title={FileTransfer},
	legend style={at={($(0,0)+(1cm,1cm)$)},legend columns=-1,fill=none,draw=black,anchor=center,align=center},
	legend to name=fred
	]

	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCPS\FTSCfilep};  
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCPS\FTSCfilep};
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCPS\FTSCfilep};  
		\addlegendentry{AdvBurst};    
	\addlegendentry{RandBurst};    

	\addlegendentry{No Attack};         
	\coordinate (c2) at (rel axis cs:1,1);% I moved this to the upper right corner
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={Precision(\%)},title={Streaming},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCPS\FTSCstreamingp};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCPS\FTSCstreamingp};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCPS\FTSCstreamingp};  
	
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={Precision(\%)},title={Torrent},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCPS\FTSCtorrentp};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCPS\FTSCtorrentp};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCPS\FTSCtorrentp};  
	
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={Precision(\%)},title={VoIP},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCPS\FTSCvoipp};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCPS\FTSCvoipp};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCPS\FTSCvoipp};  
	
	
	\end{groupplot}
	\coordinate (c3) at ($(c1)!.5!(c2)$);
	\node[below] at (c3 |- current bounding box.south)
	{\pgfplotslegendfromname{fred}};
	\end{tikzpicture}%
	\caption{The precision of FTSC-PS under different attacks over various numbers of dummy packets. The legends show the kind of attacks that have been applied to FTSC-PS.}
	\label{fig:FTSC-PS-precision}
\end{figure}


\begin{figure}[H]
	\centering
	
	\begin{tikzpicture}
	%/*
	\pgfplotsset{
		scaled y ticks = false,
		width=5cm,
		height=4cm,
		axis on top,
		%xticklabel style={text width=2em,align=center},
		%xticklabels={\empty},
		xmin=-1,xmax=21,
		ymin=-0,ymax=100,
		minor y tick num=1,
		xtick={1,3,5,7,10,12,15,17,20},
		ticklabel style = {font=\tiny},
		%xminorticks=true,
		%yminorticks=true,
		ylabel shift={-0.8em},
		ylabel style={align=center},
		xlabel shift={-0.4em},
		grid=both, 
		grid style={dashed,gray!30}
	}
	%       
	\begin{groupplot}[ 
	group style={
		group size=3 by 2,
		vertical sep=45pt,
		horizontal sep=35pt
	},
	]
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={F-score(\%)},title={Chat},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCPS\FTSCchatf};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCPS\FTSCchatf};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCPS\FTSCchatf};  

	% (Relative) Coordinate at top of the first plot
	\coordinate (c1) at (rel axis cs:0,1);
	
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={F-score(\%)},title={Email}]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCPS\FTSCemailf};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCPS\FTSCemailf};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCPS\FTSCemailf};  

	
	\nextgroupplot[
	yshift=0pt,
	xlabel={Num\_of\_Dummy\_Pkts},ylabel={F-score(\%)},title={FileTransfer},
	legend style={at={($(0,0)+(1cm,1cm)$)},legend columns=-1,fill=none,draw=black,anchor=center,align=center},
	legend to name=fred
	]

	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCPS\FTSCfilef};  
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCPS\FTSCfilef};
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCPS\FTSCfilef};  
	\addlegendentry{AdvBurst};    
	\addlegendentry{RandBurst};    

	\addlegendentry{No Attack};         
	\coordinate (c2) at (rel axis cs:1,1);% I moved this to the upper right corner
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={F-score(\%)},title={Streaming},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCPS\FTSCstreamingf};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCPS\FTSCstreamingf};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCPS\FTSCstreamingf};  

	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={F-score(\%)},title={Torrent},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCPS\FTSCtorrentf};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCPS\FTSCtorrentf};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCPS\FTSCtorrentf};  

	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={F-score(\%)},title={VoIP},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCPS\FTSCvoipf};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCPS\FTSCvoipf};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCPS\FTSCvoipf};  
	
	
	\end{groupplot}
	\coordinate (c3) at ($(c1)!.5!(c2)$);
	\node[below] at (c3 |- current bounding box.south)
	{\pgfplotslegendfromname{fred}};
	\end{tikzpicture}%
	
	\caption{The F-score of FTSC-PS under different attacks over various numbers of dummy packets. The legends show the kind of attacks that have been applied to FTSC-PS.}
	\label{fig:FTSC-PS-fscore}
\end{figure}


\begin{figure}[H]
	\centering
	
	\begin{tikzpicture}
	%/*
	\pgfplotsset{
		scaled y ticks = false,
		width=5cm,
		height=4cm,
		axis on top,
		%xticklabel style={text width=2em,align=center},
		%xticklabels={\empty},
		xmin=-1,xmax=21,
		ymin=-0,ymax=100,
		minor y tick num=1,
		xtick={1,3,5,7,10,12,15,17,20},
		ticklabel style = {font=\tiny},
		%xminorticks=true,
		%yminorticks=true,
		ylabel shift={-0.8em},
		ylabel style={align=center},
		xlabel shift={-0.4em},
		grid=both, 
		grid style={dashed,gray!30}
	}
	%       
	\begin{groupplot}[ 
	group style={
		group size=3 by 2,
		vertical sep=45pt,
		horizontal sep=35pt
	},
	]
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={Precision(\%)},title={Chat},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCIAT\FTSCchatp};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCIAT\FTSCchatp};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCIAT\FTSCchatp};  
	% (Relative) Coordinate at top of the first plot
	\coordinate (c1) at (rel axis cs:0,1);
	
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={Precision(\%)},title={Email}]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCIAT\FTSCemailp};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCIAT\FTSCemailp};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCIAT\FTSCemailp};  
	
	\nextgroupplot[
	yshift=0pt,
	xlabel={Num\_of\_Dummy\_Pkts},ylabel={Precision(\%)},title={FileTransfer},
	legend style={at={($(0,0)+(1cm,1cm)$)},legend columns=-1,fill=none,draw=black,anchor=center,align=center},
	legend to name=fred
	]

	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCIAT\FTSCfilep};  
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCIAT\FTSCfilep};
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCIAT\FTSCfilep};  
	
	\addlegendentry{AdvBurst};    
	\addlegendentry{RandBurst};    

	\addlegendentry{No Attack};         
	\coordinate (c2) at (rel axis cs:1,1);% I moved this to the upper right corner
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={Precision(\%)},title={Streaming},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCIAT\FTSCstreamingp};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCIAT\FTSCstreamingp};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCIAT\FTSCstreamingp};  
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={Precision(\%)},title={Torrent},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCIAT\FTSCtorrentp};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCIAT\FTSCtorrentp};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCIAT\FTSCtorrentp};  
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={Precision(\%)},title={VoIP},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCIAT\FTSCvoipp};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCIAT\FTSCvoipp};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCIAT\FTSCvoipp};  

	
	\end{groupplot}
	\coordinate (c3) at ($(c1)!.5!(c2)$);
	\node[below] at (c3 |- current bounding box.south)
	{\pgfplotslegendfromname{fred}};
	\end{tikzpicture}%
	
	\caption{The precision of FTSC-IAT under different attacks over various numbers of dummy packets. The legends show the kind of attacks that have been applied to FTSC-IAT.}
	\label{fig:FTSC-IAT-precision}
\end{figure}


\begin{figure}[H]
	\centering
	
	\begin{tikzpicture}
	%/*
	\pgfplotsset{
		scaled y ticks = false,
		width=5cm,
		height=4cm,
		axis on top,
		%xticklabel style={text width=2em,align=center},
		%xticklabels={\empty},
		xmin=-1,xmax=21,
		ymin=-0,ymax=100,
		minor y tick num=1,
		xtick={1,3,5,7,10,12,15,17,20},
		ticklabel style = {font=\tiny},
		%xminorticks=true,
		%yminorticks=true,
		ylabel shift={-0.8em},
		ylabel style={align=center},
		xlabel shift={-0.4em},
		grid=both, 
		grid style={dashed,gray!30}
	}
	%       
	\begin{groupplot}[ 
	group style={
		group size=3 by 2,
		vertical sep=45pt,
		horizontal sep=35pt
	},
	]
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={F-score(\%)},title={Chat},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCIAT\FTSCchatf};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCIAT\FTSCchatf};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCIAT\FTSCchatf};  
	% (Relative) Coordinate at top of the first plot
	\coordinate (c1) at (rel axis cs:0,1);
	
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={F-score(\%)},title={Email}]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCIAT\FTSCemailf};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCIAT\FTSCemailf};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCIAT\FTSCemailf};  
	
	\nextgroupplot[
	yshift=0pt,
	xlabel={Num\_of\_Dummy\_Pkts},ylabel={F-score(\%)},title={FileTransfer},
	legend style={at={($(0,0)+(1cm,1cm)$)},legend columns=-1,fill=none,draw=black,anchor=center,align=center},
	legend to name=fred
	]

	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCIAT\FTSCfilef};  
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCIAT\FTSCfilef};
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCIAT\FTSCfilef};  

	\addlegendentry{AdvBurst};    
	\addlegendentry{RandBurst};    
	\addlegendentry{No Attack};         
	\coordinate (c2) at (rel axis cs:1,1);% I moved this to the upper right corner
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={F-score(\%)},title={Streaming},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCIAT\FTSCstreamingf};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCIAT\FTSCstreamingf};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCIAT\FTSCstreamingf};  
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={F-score(\%)},title={Torrent},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCIAT\FTSCtorrentf};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCIAT\FTSCtorrentf};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCIAT\FTSCtorrentf};  
	\nextgroupplot[ xlabel={Num\_of\_Dummy\_Pkts},ylabel={F-score(\%)},title={VoIP},]
	\addplot[\colorone,mark=\markone,mark size=1.0]    table[x=AdvBurstOverHead,y=rand,col sep=comma]{\FTSCIAT\FTSCvoipf};
	\addplot[\colortwo,mark=\marktwo,mark size=1.0]    table[x=AdvBurstOverHead,y=AdvBurst,col sep=comma]{\FTSCIAT\FTSCvoipf};  
	\addplot[only marks,\colorfive,mark=\markfive]    table[x=AdvBurstOverHead,y=natural,col sep=comma]{\FTSCIAT\FTSCvoipf};  
	
	
	\end{groupplot}
	\coordinate (c3) at ($(c1)!.5!(c2)$);
	\node[below] at (c3 |- current bounding box.south)
	{\pgfplotslegendfromname{fred}};
	\end{tikzpicture}%
	
	\caption{The F-score of FTSC-IAT under different attacks over various numbers of dummy packets. The legends show the kind of attacks that have been applied to FTSC-IAT.}
	\label{fig:FTSC-IAT-fscore}
\end{figure}


==> content/related_old.tex <==
%Statistical Traffic classification has been widely studied in the network management domain with three major approaches, Packet classification, Flow Content Classification and Flow Time series Classification.In Some of The applications such as SDN and QoS it is needed to be decide how each packet routed. in this circumstances classifier came to facilitate the process of network management.


%In Some cases such as anonymity networks, content of packets are obfuscated and no valuable information can be extracted from content of packets furthemore in some cases privacy preserving of users is a priority and thus researcher prefer to use statistical feature of flows instead of flow content. Statistical features like Direction, Inter arrival time and packet sizes are among the most significant features.

The DL-based network traffic classification has been widely studied in the literature, and a brief review of previous studies has been provided in this section. Based on the category of input space, the studies is explained in separate sections. Table \ref{tab:RW} provides an overview of previous studies.

\subsection{Packet Classification}

Lotfollahi et al. present the Deep Packet framework that embeds stacked autoencoder and convolutional neural networks to classify network traffic \cite{DBLP:journals/soco/LotfollahiSZS20}. Their framework reduces manual efforts for feature engineering, and they claim that the Deep packet outperform all of the similar works on the ISCXVPN2016 dataset. The Deep Packet uses the byte sequence of the transport layer header and the payload of packets to classify packets. Regarding their claim, this work is the first try to perform both application identification and traffic characterization by a DL-based classifier. The results show that the 1D-CNN classifier has better overall performance rather than SAE in both application identification and traffic characterization, and the overall accuracy of the 1D-CNN in application identification is 0.98\%, and the precision in traffic characterization is 93\%.

Wang et al. introduce a DL based encrypted traffic classifier called Datanet for better management of distributed smart home networks and aiding the software-defined-network (SDN) controller in real-time network traffic monitoring and classification \cite{DBLP:journals/access/WangYCQ18}. In the first step, packets are preprocessed, and after removing the header of the Data-link layer, the byte sequence of packets is fed to the Datanet. 
Same as \cite{DBLP:journals/soco/LotfollahiSZS20}, Datanet uses the ISCXVPN2016 dataset and reaches the F-measure of ≥ 96\% for both the SAE and CNN in distinguishing 15 applications.

\subsection{Flow Content Classification}
The first method to apply deep learning in traffic classification is introduced by Z. Wang et al. \cite{wang2015applications}. They recognize remarkable feature engineering ability of deep learning and try to detect protocols in the TCP flow dataset by means of SAE. Their dataset consists of 300k pre-processed records in which exist 1000 bytes of TCP payload. They achieve more than 90\% recall in protocol detection for all protocols.

W. Wang et al. propose an end-to-end encryption traffic classifier for traffic characterization \cite{DBLP:conf/isi/WangZWZY17}. They use the ISCXVPN2016 dataset and extract only 728 bytes of each flow as the input. The authors have shown that the 1D-CNN has better performance rather than 2D-CNN in network traffic classification. Also, they investigate the influence of headers and the type of flows in network traffic classification. The result of their study shows that including headers in the input improves the performance of the network traffic classifier, and the classifier has better performance on bidirectional flows rather than unidirectional flows. They achieve the best result in the classification of the ISCXVPN2016 dataset compared to previous works that use the classical ML algorithms. 
In another work, they identify malware traffic using the same approach, by transforming raw traffic data to image and using 2D-CNN as the spatial feature learner \cite{DBLP:conf/icoin/WangZZYS17}.

After several studies in the domain of mobile application identification \cite{DBLP:journals/tifs/TaylorSCM18,DBLP:conf/eurosp/TaylorSCM16}, Aceto et al. addressed mobile application identification through the Deep Learning approach \cite{DBLP:journals/tnsm/AcetoCMP19} for the first time. They investigate the type of input data that is fed to the DL-classifier and consider three types of input data: ($i$) first N bytes of payload in a flow, ($ii$) first N bytes of all headers and payloads in a flow, and ($iii$) source and destination ports, number of bytes in the transport-layer header, TCP window size, inter-arrival time, and direction of packets in a flow. 
While the results demonstrate the classifier, which is trained on the second type of input data, has the best performance, the authors claim that the results of the classifier are biased to the information in headers and hence not meaningful. The performance of the classifier is trained on the first type of input data is better than the classifier is trained on the third type of input data, and they achieve 83\% overall accuracy for identifying 45 applications in both Android and IOS operating systems. Also, they demonstrate that the overall performance of 1D-CNN and 2D-CNN are close in mobile application identification and suggest that traffic should be extracted by naturally considering data as one-dimensional. 

\subsection{Flow Time Series Classification}
In \cite{DBLP:conf/icissp/Draper-GilLMG16}, authors utilize a set of time-related features such as duration of flow, byte per second, and inter-arrival time between packets for network traffic classification. They use C4.5 and K-nearest neighbors as classification techniques and achieve about 80\% accuracy in the characterization of network traffics. Moreover, they generate and distribute a labeled dataset of encrypted network traffic called ISCXVPN2016, which became a criterion in network traffic classification.

In \cite{DBLP:journals/cn/Caicedo-MunozEC18} authors improve the performance of \cite{DBLP:conf/icissp/Draper-GilLMG16}, and achieve about 83\% accuracy on the ISCXVPN2016 dataset using bagging and boosting classifiers. Since these two studies use the time-related features of the entire flow to classify network traffic, their approaches are not useful in online policy enforcement systems.

Rezaei and Liu propose a semi-supervised approach based on a 1D-CNN to classify five Google applications \cite{DBLP:journals/corr/abs-1812-09761}. They train a 1D-CNN to predict the statistical features of the entire flow from a few sampled packets on a large unlabeled dataset. Then, they transfer the 1D-CNN to a new classifier and add some fully connected layers to the top of it. Afterward, the new classifier re-train on a few labeled samples for application identification task. They show the possibility of using sampled packets features instead of first n packets in network traffic classification, which is more feasible for high bandwidth operational networks.

Lopez-Martin et al. \cite{DBLP:journals/access/MartinCSL17} introduce a new hybrid classifier based on CNN and RNN to detect services used by different devices with various user-profiles in IoT network traffic. In this work, each flow comprises 20 packets, and each packet contains six features, including source port, destination port, the number of bytes in the packet payload, TCP window size, inter-arrival time, and direction of packets. Regarding the results, whenever the RNN is combined with a CNN, success rate slightly improves, and the performance of the classifier decreases by including inter-arrival times in the input.

The process of identifying visited websites through anonymized traffic, which is also known as Website Fingerprinting (WF), has a background as long as encrypted traffic classification. Abe and Goto investigate the effectiveness of DL-based classifiers in WF for the first time \cite{abe2016fingerprinting}. They reveal that SAE is useful in the detection of 100 websites that are sent trough Tor with an 86\% success rate.

Rimmer et al. indicate that DL is an effective tool in automating the process of features engineering, and it can eliminate the need for feature design and selection. Their SAE achieves a 95.3\% success rate only using the direction of Tor packets (Tor cells) \cite{DBLP:conf/ndss/RimmerPJGJ18}. In another work, Sirinam et al. design a deeper CNN classifier to outperform earlier works, which increase the success rate to 98\% \cite{DBLP:conf/ccs/SirinamIJW18}. These works indicate that applying deep learning reduces the reliance on human insight for feature engineering, as well as notable improvement in the performance of WF classifiers.


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
	\caption{Overview of previous studies.}
	\label{tab:RW}
	\setlength\extrarowheight{5pt}
		\resizebox{16cm}{!}{%
	\begin{tabular}{|c|ccccc|}
		\hline
		\rowcolor[HTML]{EFEFEF} 
		\begin{tabular}[c]{@{}c@{}}Input Space\\ Category\end{tabular} & Paper                                                                 & Input data                  & Classifier        & Classification Target             & Year \\ \hline
		\cellcolor[HTML]{EFEFEF}                                       & P. Wang et al. \cite{DBLP:journals/access/WangYCQ18}                 & $H^{IP}$,$H^{TL}$,$payload$             & SDAE,MLP,CNN   & Application identification        & 2018 \\
		\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}PC}                   & M. Lotfollahi et al. \cite{DBLP:journals/soco/LotfollahiSZS20}        & $H^{TL}$,$payload$                 & SAE,CNN       & \begin{tabular}[c]{@{}c@{}}Application identification,\\ Traffic characterization \end{tabular}  & 2017 \\ \hline
		\cellcolor[HTML]{EFEFEF}                                       & Z. Wang et al. \cite{wang2015applications}            & $H^{TL}$,$payload $                  & SAE               & Protcol detection                 & 2015 \\
		\cellcolor[HTML]{EFEFEF}                                       & W. Wang et al. \cite{DBLP:conf/isi/WangZWZY17}                     & $H^{IP}$,$H^{TL}$,$payload$                 & CNN               & Traffic characterization          & 2017 \\ 
				\multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}FCC} 
		\cellcolor[HTML]{EFEFEF}                                       & W. Wang et al. \cite{DBLP:conf/icoin/WangZZYS17}                 & $H^{IP}$,$H^{TL}$,$payload$              & SAE               & Malware classification            & 2017 \\ \hline
            				\multirow{-1}{*}{\cellcolor[HTML]{EFEFEF}FCC-FTSC}    & G. Aceto et al. \cite{DBLP:journals/tnsm/AcetoCMP19}                &\begin{tabular}[c]{@{}c@{}}$H^{IP}$,$H^{TL}$,$payload$,\\ $IAT$,$PS$,$Dir$\end{tabular}                    & SAE,CNN          & Application identification        & 2019 \\ \hline
		\cellcolor[HTML]{EFEFEF}                                       & J. Caicedo-Muñoz et al. \cite{DBLP:journals/cn/Caicedo-MunozEC18}        & Time-related features       & Bagging, Boosting & Traffic characterization          & 2018 \\ 
		\cellcolor[HTML]{EFEFEF}                                       & G. Draper-Gi et al. \cite{DBLP:conf/icissp/Draper-GilLMG16} & Time-related Features       & KNN,C4.5         & Traffic characterizaion           & 2016 \\
		\cellcolor[HTML]{EFEFEF}                                       & M. L{\'{o}}pez Mart{\'{\i}}n et al. \cite{DBLP:journals/access/MartinCSL17}           & $PS$,$Dir$,$H^{TL}$  & LSTM,CNN          & Protcol detection                 & 2017 \\
		\cellcolor[HTML]{EFEFEF}                                       & K. Abe And S. Goto \cite{abe2016fingerprinting}                             & $Dir$,$IAT$         & SDAE              & Website classification            & 2016 \\
		\cellcolor[HTML]{EFEFEF}                                       & V. Rimmer et al. \cite{DBLP:conf/ndss/RimmerPJGJ18}                        &  $Dir$     & SDAE,CNN,LSTM    & Website classification            & 2017 \\
		\cellcolor[HTML]{EFEFEF}                                       & P. Sirinam et al. \cite{DBLP:conf/ccs/SirinamIJW18}                      &  $Dir$     & CNN               & Website classification            & 2018 \\
		\multirow{-7}{*}{\cellcolor[HTML]{EFEFEF}FTSC}                 & S. Rezaie and X. Liu \cite{DBLP:journals/corr/abs-1812-09761}                & $IAT$,$PS$,$Dir$           & CNN               & Application identification        & 2018 \\ \hline
	\end{tabular}
}
\end{table}


